4D Spatio-Temporal Convolutional Networks for Object Position Estimation in OCT Volumes

Tracking and localizing objects is a central problem in computer-assisted surgery. Optical coherence tomography (OCT) can be employed as an optical tracking system, due to its high spatial and temporal resolution. Recently, 3D convolutional neural networks (CNNs) have shown promising performance for pose estimation of a marker object using single volumetric OCT images. While this approach relied on spatial information only, OCT allows for a temporal stream of OCT image volumes capturing the motion of an object at high volumes rates. In this work, we systematically extend 3D CNNs to 4D spatio-temporal CNNs to evaluate the impact of additional temporal information for marker object tracking. Across various architectures, our results demonstrate that using a stream of OCT volumes and employing 4D spatio-temporal convolutions leads to a 30% lower mean absolute error compared to single volume processing with 3D CNNs.

==> README <==
                 The dgruyter package:                 
preparing books and journals for Walter de Gruyter GmbH


File:       README
Author:     le-tex publishing services


DESCRIPTION
===========

The dgruyter package assists in preparing manuscripts for de Gruyter
with {\LaTeX}. It provides some special commands for journal papers
as well as for books and generates the required appearance.
Together with corresponding font packages it allows to produce the 
final layout of De Gruyter books and journal articles.

Copyright:  (C) 2015, 2016, 2017 Walter de Gruyter GmbH


FILES IN DISTRIBUTION
=====================

   BASE DISTRIBUTION:

      README                  This file.
      dgruyter.ins            Package installation file.
      dgruyter.dtx            Package source file.
      dg-degruyter.eps/.pdf   Logo files.
      dg-mouton.eps/.pdf      Logo files.
      dg-saur.eps/.pdf        Logo files.
      DG_attention.eps/.pdf   Vignette files.
      DG_exercise.eps/.pdf    Vignette files.
      DG_information.eps/.pdf Vignette files.
      DG_notice.eps/.pdf      Vignette files.
      DG_question.eps/.pdf    Vignette files.
      book.tex                Template file for a book.
      article.tex             Template file for a journal article.
      issuetoc.tex            Template file for a journal issue toc.


   DOCUMENTATION:

      dgruyter.pdf            User manual for dgruyter package. 
                              It is produced as described below.


BASIC INSTALLATION
====================

   To get the package style file 'dgruyter.sty' and the
   index style files 'dgruyter.ist' and 'dgruyter.xdy' execute:
     latex dgruyter.ins

   The minimum requirement to use the package is to have
     dgruyter.sty and dgruyter.ist/dgruyter.xdy
     (as well as the logo and vignette files)
     in a directory where TeX can find it.

   To get the documentation 'dgruyter.pdf' execute:
     pdflatex dgruyter.dtx (at least twice)

